Towards Concolic Testing for Hybrid Systems

Hybrid systems exhibit both continuous and discrete behavior. Analyzing hybrid systems is known to be hard. Inspired by the idea of concolic testing (of programs), we investigate whether we can combine random sampling and symbolic execution in order to effectively verify hybrid systems. We identify a sufficient condition under which such a combination is more effective than random sampling. Furthermore, we analyze different strategies of combining random sampling and symbolic execution and propose an algorithm which allows us to dynamically switch between them so as to reduce the overall cost. Our method has been implemented as a web-based checker named HyChecker. HyChecker has been evaluated with benchmark hybrid systems and a water treatment system in order to test its effectiveness.

==> sec-commentout.tex <==
%the below paragraphs are commented, in case we don't have the swat model by then.
%the below paragraphs are commented, in case we don't have the swat model by then.
%the below paragraphs are commented, in case we don't have the swat model by then.
%the below paragraphs are commented, in case we don't have the swat model by then.
%the below paragraphs are commented, in case we don't have the swat model by then.
%the below paragraphs are commented, in case we don't have the swat model by then.
\iffalse
\subsection{The IWA Open Benchmark Model}
This activated sludge process aims to achieve low concentration of biodegradable matter in the effluent together with minimal sludge production \cite{iwamanual} .
\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{image/iwalayout}
	\caption{The Schematic Layout of BSM1}
	\label{piciwalayout}
\end{figure}

Let's take a look at the schematic layout of the simulation benchmark in Fig. \ref{piciwalayout}, this layout has 5 biological tanks-in-series with a secondary settler. The influent goes into tank 1, and the waste water from tank 5 will go back to influent for recycling purposes. Clean water would go out from the settler. The layout consists of two models simultaneously: the biological process model and the settling process model. The former model contains 13 state variables and 8 processes, the latter contains a settling velocity equation for each kind of solid matter.

This example contains two control loops, the first loop involves controlling the dissolved oxygen level in the final compartment by manipulation of the oxygen transfer coefficient, the second control loop involves controlling the nitrate level in the second tank by manipulation of the internal recycle flow rate. For different parameters set, comes in multiple modes in our hybrid automata model.
This model is straightforward as the parameters to manipulate are only two but modes would be multiple as the combination of the two parameters are plenty. I will use this benchmark as a demo of our concolic verification method. While this model is based on an open benchmark out of which anyone could design their own model, the SWaT model is based on a more realistic and complicated facility.

\subsection{The SWaT Model}
This system in Fig. \ref{watersystem} is a simulation of a real water purification system located at Singapore University of Technology and Design. The system consists of 7 phases, each could be modeled tested separately. There are more than 50 sensors in this system, which means we have at least 50 state variables and hence a lot of equations.
\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{image/watersystem}
	\caption{The Schematic Layout of BSM1}
	\label{watersystem}
\end{figure}
As talked in previous section, I need to model this in OOP, dividing the functions in 4 different modules. I'm modeling this system in LabView and python. As shown in Fig. \ref{modules}, the PLC codes in C are provided by vendors, every new parameter reassigned by the PLC means the system is going into different modes, thus in our hybrid automata, we divide different modes based on the control logic. The information of the sensor and actuators are also provided by the vendors while I need to do mathematical abstraction of behavior of the devices, writing them in ODEs.

The most difficult part is to mathematically abstract the processes. The processes could be as simple as modeling the filling of tanks, or as complicated as depicting the chemical reactions, which wouldn't be easy task even for experts in chemistry. So I'm thinking of machine learning techniques. To do this, I need massive data to train my models, and the trained models might not be entirely written in ODEs, I need to undergo further work on this.



\subsection{PID Control}
PID control is widely used in computer controlled systems. The general form is in equation \ref{pidcontrol}. Here $e(t)=Real(t)-Set(t)$ stands for error, where $MV(t)$ is the output value of the PID controller. $Kp$, $Ki$ and $Kd$ are proportional, integral and derivative gain respectively. As a negative feedback controller, PID controller helps to retain the real value around the set values.

\begin{equation}
MV(t)= {K_p}e(t)+{K_i}\int_{0}^{t}e(\tau )d\tau +{K_d}\frac{d}{dt}e(t)
\label{pidcontrol}
\end{equation}

To avoid introducing PDEs to our system, or in other words, to require our system to be time-invariant, which means that for same input value at different time points, the system will always generate the same value. I will drop the integration part, as solving this part will involve PDE solver, and it is not supported in hybrid automata. By assigning 0 to $Ki$, we get a PD controller, we have 6 controllers in our system, altogether they decide the behavior of the system based on different inputs.

\subsection{ODE Solver and Rare Event}
ODE solvers are crucial for the random simulation of hybrid automata which are based on various algorithms which are specified for certain ODE formats. Inappropriate solvers chosen will cause errors, as time advances, the simulation results will grow more untrustworthy. In here, after building the model, I need to test different solvers for their accuracy and simulation time consumption. The solvers are also divided into 2 categories based on simulation step size, one is constant step size, the other is variant step size. No matter which kind to use, it is easy to come across a so called rare-event situation. Rare events are events that has very little possibility of happening. While once happen, will fulfill the jump condition to a new mode from current one. If the simulation step size is not small enough or when we use a constant step size for simulation and the period of the event happening is the same or times of that of the step size, then this jump condition would never be noticed by the hybrid automata. One way is to change the step size to variant, the other is to call dReal to symbolically find a path.

To instantiate, take a look at the the input water flow which rushes very high and falls down quickly, causing the water tank level to rise and fall between two simulation time points. In real system, this will trigger the emergency valve to open, discharging surplus water and in the meantime, stop the inflow until a new guard is satisfied and system jumps away from the current mode. This event will obviously make a huge change to the system state. While in traditional simulation methods, this kind of event could hardly be noticed, and the simulation would go far wrong. As mentioned in the system overview, to trigger the rare event, we adjust the input flow, adding a new function to the original flow function. In equation \ref{rareinput}, we depict the input flow wave. The trigonometric function is the normal input, and the latter part denotes a flow rush, which gets its largest value $C_{2}$ when $ t=b $, and with smaller $a$, comes smaller noticeable interval for this event. This situation has realistic meanings. As in the open benchmark of the IWA model, we would come across a storm or a extremely dry weather.

\begin{equation}
in\_flow(t)=C_{1}sin(\omega t)+C_{2}e^{-\frac{(t-b)^{2}}{a}}
\label{rareinput}
\end{equation}
\fi
%the above paragraphs are commented, in case we don't have the result of swat MODEL by then.
%the above paragraphs are commented, in case we don't have the result of swat MODEL by then.
%the above paragraphs are commented, in case we don't have the result of swat MODEL by then.
%the above paragraphs are commented, in case we don't have the result of swat MODEL by then.
%the above paragraphs are commented, in case we don't have the result of swat MODEL by then.
%the above paragraphs are commented, in case we don't have the result of swat MODEL by then.
%the above paragraphs are commented, in case we don't have the result of swat MODEL by then.
%the above paragraphs are commented, in case we don't have the result of swat MODEL by then. 


==> sec-conclusion.tex <==
\section{Conclusion}\label{conclusion}
In this work, we investigated the effectiveness of different sampling methods (i.e., random sampling and symbolic execution) for hybrid systems. We established theoretical results on comparing their effectiveness and more relevantly we developed an approach for combining random sampling and symbolic executions in a way which is provably cost-effective. 





==> sec-evaluation.tex <==
\section{Evaluation of Experiment Results}





In the room heating system, we assert the heat will eventually move in the $5$ day period, where the random testing method was not able to find.
In the navigation benchmark, we are also able to assert that the grid $A$ is reachable. In transportation safety testing, this could be very useful results.
In the SWaT system, we are able to find that the backwash tank could overflow or drain off given the range of the initial conditions. And in turn shut down the whole system.
Generally, our tool \emph{HyChecker} is able to spot counterexamples quicker compared to the random testing algorithm given same computing budget.



==> sec-hybridautomata.tex <==
\section{Detailed Approach} \label{sec:ha}



Figure~\ref{bouncing_ball} shows a simple example of hybrid systems: a bouncing ball system. The bouncing ball system uses a scalar $v$ to indicate the absolute speed of the ball and a scalar $x$ to indicate the height of the ball. Variables $v$ and $x$ are called \emph{state variables} of the system. When the ball is falling, the speed $v$ increases and the height $x$ decreases by the rate of $v$. This fact is captured by the mode \emph{falling down} with ordinary differential equations
\begin{equation*}
\left\{
\begin{aligned}
\dot{v} &= g, \\
\dot{x} &= -v.
\end{aligned}
\right.
\end{equation*}

Similarly we have another mode \emph{bouncing back} to indicate when the ball is bouncing back to its highest point. When the ball hits the ground, the bouncing ball system immediately jumps from mode ``falling'' to ``bouncing''; when the ball reaches its highest, it jumps from mode ``bouncing'' to ``falling''.

We will introduce our method on the model of hybrid automata, but our method is not constrained within hybrid automata and can be generalized to other formal models, such as hybrid CSP \cite{liu2010calculus}, hybrid event-B \cite{banachcore}.



==> sec-illustrative.tex <==
\section{A Running Example} \label{example}
In this section, we use a \emph{sewerage system} as a toy example to illustrate how {\HC} works. The system controls the water flow to maintain the inward water level within a safe region. The system stays in the \emph{normal} mode as long as the water flow is within a safety range. Otherwise, the system jumps to \emph{draining} (or \emph{loading}) mode. In case of a storm, the system should notice the dramatic increase of water level in a short time and set a flooding alarm. We remark that storms are the \emph{rare events} in this example.

In this work, we model the systems as hybrid automata~\cite{alur1993hybrid}, which are designed to model hybrid systems. Figure~\ref{SewerageSystem} shows the hybrid automaton modeling the system. The circles denote different system modes and the transitions denote mode changes. A hybrid automaton is associated with a set of continuous state variables. Each mode is associated with a set of ordinary differential equations, which specifies how the state variable evolve through time in the mode.
%%%sunjun: you need to explain why we use this formula; the formula is for which mode and what are the formula for other modes? What are the transition guards?
For instance, in this example, there is a continuous variable $x$ which models the dynamics of the water flow. At mode $normal$, $x$ evolves according to the following differential equation.
$$
\frac{\mathrm{d}x}{\mathrm{d}t} = -\frac{M(t - \mu)}{\sigma ^2} \exp\left(-\frac{(t-\mu)^2}{2\sigma^2}\right) + m\omega \cos(\omega t),
$$
According to the equation, most of the time, the flow is within a normal range $[-m,m]$. However during a very short time period the flow may dramatically increase to $M$, as shown in Figure~\ref{storms}.
%%%sunjun: from the figure, it seemed that the function is not continuous? what is M in this case? and other constants?

Transitions in hybrid automata are guarded by propositional logic formulae. For instance, in the above example, the transition from mode $normal$ to $draining$ is guarded by $x \textgreater 8$, where the transition from $normal$ to $flooding$ is guarded by $x \textgreater 37$.

\begin{figure}[t]
\centering
\scalebox{0.8}{
\begin{tikzpicture}[->, node distance = 3cm,scale = 1]
	\tikzstyle{every node} = [align = center,minimum size = 1 cm];
	\node [initial by arrow,initial text=,initial where = above,state] (INIT){normal};
	\node [state](T1)[left of = INIT]{draining};
	\node [state](T2)[right of = INIT]{loading};
	\node [state,draw=red](T3)[below of = INIT]{flooding};%this is a rare mode
	\node [state](T4)[left of = T3]{recover};
	\node [state](T5)[right of = T3]{shutdown};
	\path
		(INIT)edge[bend left]node [above=0.01cm] {$x>8$}(T1)
		(INIT)edge[bend left] node [above=0.01cm] {$x<2$}(T2)
		(INIT)edge[draw=red] node [right=0.01cm]{$x>37$}(T3)
		(T1)edge[bend left] node [above=0.01cm] {$x<8$}(INIT)
		(T2)edge[bend left] node [above=0.01cm] {$x>2$}(INIT)
		(T3)edge[] node [above=0.01cm] {$x\times t > 37$}(T4)
		(T3)edge[] node [above=0.01cm]{$x\times t < 28$}(T5)
		(T4)edge[] node [left=0.01cm] {$x < 12$}(INIT);
\end{tikzpicture}
}
\caption{A sewerage system with rare events}
	\label{SewerageSystem}
\end{figure}

When the mode of $flooding$ is entered, the sewerage system opens the emergent draining pipe, and the ODE in this mode is as depicted below.
$$
\frac{\mathrm{d}x}{\mathrm{d}t} = -\psi \ flow + m\omega \cos(\omega t),
$$
Intuitively, the higher the flow, higher the drain off speed. While at this mode, the future system behavior of the system depends on the value of the drain off speed $\frac{\mathrm{d}x}{\mathrm{d}t}$. If $-\psi \ x + m\omega \cos(\omega t) \textgreater 37$, the system enters the $shutdown$ mode as the drain off speed exceeds the system's limit. If $-\psi \ x + m\omega \cos(\omega t) < 28$, the system goes to the $recover$ mode, as the emergent draining is no longer needed.
%%%sunjun: the text and the figure are inconsistent. 
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.4\textwidth]{image/bouncing_ball.png}
%	\hspace{10pt}
%	\begin{tikzpicture}[->, node distance = 2cm]
%		% tikzstyle
%		\tikzstyle{every node} = [align = center,minimum size = 2cm];
%		\node [state] (UP) {$\dot{v}=-g$\\$\dot{x}=-v$};
%		\node [initial, state]	(DOWN) [above left of = UP] {$\dot{v}=g$\\$\dot{x}=v$};
%		\path
%			(UP) edge [bend left, left] node {$v = 0$} (DOWN)
%			(DOWN) edge [bend left, right] node {$x = 0$} (UP);
%	\end{tikzpicture}
%	\caption{Dynamic Behavior and Hybrid Automata of \emph{Bouncing Ball}}
%	\label{bouncing_ball}
%\end{figure}

For simplicity, we assume that the property that we are checking in is whether it is true that mode $shutdown$ is never reached. We apply first a sampling method similar to the one proposed in~\cite{benjaminsmc} and quickly discover that mode \emph{draining} and \emph{loading} are reachable. However, obtaining a sample reaching mode $shutdown$ is not always easy. On the XXth simulation, the transition from $normal$ to $flooding$ is fired. Continuing the simulation, it seemed that the transition is fired only on average once of XXX simulations. Furthermore, after XXX simulation, the transition from $flooding$ to $shutdown$ is still not fired. The question is then, do we continue with the sampling, with the hope that a counterexample will be sampled soon, or do we switch to an alternative method like symbolic execution (i.e., encoding and solving the path condition from $normal$ to $shutdown$)? %To answer this question formally, we need to know what is the probability of sampling a counterexample (e.g., what is the expected number of samples) and, with the knowledge on the cost of generating each sample, compare the cost of identifying the counterexample through sampling and the cost of solving the path condition.
As far as we know, this question is not answered systematically in previous approaches.

\textsc{HyChecker} works as follows for this example. Initially, with no knowledge on the probability of each transition occurring in the system model, \textsc{HyChecker} builds a probabilistic model where //TODOFirstly, a simulation is generated using the approach in~\cite{benjaminsmc}. For instance, the simulation goes through the following sequence of modes: $\langle \rangle$. Based on the simulation result, \textsc{HyChecker} builds its first estimation of the

%%%sunjun: explain here how our algorihtms works step by step. Do not explain too much on the technical details of the steps, just the result and perhaps some intuition why.
 
% Table~\ref{methodcomparison} column 2 shows our experiments (with 10 trials using the method in~\cite{benjaminsmc}) and only once out of 10 experiments we are able to show that $flooding$ is reachable. On the contrary, our approach {\HC} reaches a higher coverage rate~(Table~\ref{methodcomparison}, Column~1). It first applies random sampling until no new unreached modes is discovered. Then {\HC} turns to an SMT solvers (i.e., dReach) to symbolically check if any reachable modes are missed. If it is the case, the SMT solvers will return an \emph{importance region} which will lead the system to an undiscovered mode for sure. \HC will adjust the sampling distribution and cast more emphasis on the importance region by applying the method of \emph{importance sampling}.



\begin{figure}[t]
\centering
\includegraphics[scale = 0.30]{image/sewe_flood_full.png}
\caption{Storms come in a very short period of time}
\label{storms}
\end{figure}


%We tested this example system with two methods: {\HC} against random sampling. Results are collected in Table~\ref{methodcomparison}. As we expected, random sampling has a good efficiency but does not work well when systems contain rare events. In fact, it fails nine times out of ten to detect the coming storm, for the flooding does come in a flash.  The method of importance sampling that {\HC} uses balances the advantages and disadvantages of random sampling and pure concolic testing by SMT solvers. It successfully detected the storm in less time than random sampling.

%This toy example illustrates the power of importance sampling that it is able to find rare events which random sampling can hardly find.

%Our $INIT$ mode depicts the behavior of sewerage water flow. The ODE is shown in Eq. \ref{deriflow}. If flow exceeds threshold $thre\_high$, the hybrid system would jump to $mode\ 1$ with more pipes open. If flow falls below threshold $thre\_low$, the hybrid system would jump to $mode\ 2$ with pipes closed. However, when storms come, the water flow would increase to a high value extremely quickly and exceed $thre\_storm$, and the system should jump to $modzhe\ 3$ with emergent drain off scheme. The time span of storm is very short, and we consider it as our \emph{rare\ event}.

%\begin{equation}\label{deriflow}
%\frac{\mathrm{d}flow}{\mathrm{d}t} = -\frac{t - \mu}{\sigma ^2}\ m_s\ exp(-\frac{(t-\mu)^2}{2\sigma^2}) + \omega\ m_n\ cos(\omega t)
%\end{equation}
%
%To explicitly analyze the system, we firstly solve out the primitive function in closed form as shown in Eq. \ref{primflow}. $flow_{t=0}$ is our initial value of $flow$.
%
%\begin{equation}\label{primflow}
%flow = m_s\ exp(-\frac{(t-\mu)^2}{2\sigma^2}) + m_n\ sin(\omega t)+flow_{t=0}
%\end{equation}
%
%Then we write our guard towards $mode\ 3$ in Eq. \ref{guardrare}, through which we can tell that the solution region is approximately $(\mu-\sigma,\mu+\sigma)$. And for settling the parameter $\sigma$, we define $4\sigma$ as the time ratio of the storm event, which is $10\ min$ in our setting. For convenience, we normalize the region $(0,24)\ hour$ down to $(0,1)$. According to our calculation, in random testing the sample rate $J$ should exceed $288$ in order to surely find the region satisfying guard $3$.
%
%\begin{equation}\label{guardrare}
%flow \geq thre\_storm\\ = m_s\ exp(-\frac{(-\sigma)^2}{2\sigma^2}) + flow_{t=0}
%\end{equation}
%
%The parameters were set as follows. Time step $dt$ was set to be $1$, total sample rate $J$ is set to $10$, the $max\_len$ was set to $3$. Thus the BLTL formula we tested were shown in Eq. \ref{seweragebltl}.
%\begin{equation}\label{seweragebltl}
%\square (\neg (mode\ 2))
%\end{equation}
%
%We provide parameter settings for \emph{HyChecker} so that it can run in both importance sampling mode and in pure random testing mode. We did $10$ experiments for the sewerage system with the BLTL formula in Eq. \ref{seweragebltl}. Our results are shown in Table. \ref{methodcomparison}. As can be seen, importance sampling mode were able to give the False assertion in 9 of the total 10 runs, while we only failed once with importance sampling. As for pure random sampling, we got the True assertion for 9 runs, which means that the pure random mode were not able to discover the rare guard. We only got the False assertion for 1 run.
%
%Note that our algorithm involves randomness, so the time consumption and result could differ between different runs.



%
%\begin{table}[t]
%\centering
%\setlength{\tabcolsep}{7pt}
%\begin{center}
%\begin{tabular}{ccc}
%Tests & \multicolumn{2}{c}{Flooding detected? / Time (sec)} \\
%\hline
%% & \multicolumn{2}{c}{Methods}\\
%\cline{2-3}
%        &\HC & Random Sampling\\
%\hline
% 1&  Yes / 2.7 &  No / 623.4  \\
% 2&  No / 21.5 & No / 624.3  \\
% 3&  Yes / 13.3 & No / 667.9  \\
% 4&  Yes / 5.7 & Yes / 404.1  \\
% 5&  Yes / 2.7 & No / 666.2  \\
% 6&  Yes / 2.8 & No / 650.8  \\
% 7&  Yes / 3.9 & No / 648.2  \\
% 8&  Yes / 4.5 & No / 657.9  \\
% 9&  Yes / 6.8 & No / 650.6  \\
% 10&  Yes / 4.1 & No / 653.3  \\
%\end{tabular}
%\end{center}
%\caption{Sewerage system checking outcome }
%\label{methodcomparison}
%\end{table}


%We also tested in pure random sampling method with $J$ to be $100$, and the algorithm gave the False assertion to the tested BLTL property, which fulfills our expectation. However, though this assertion is correct, the time consumption is $2509.2$ second. It's generally much longer than the importance sampling method.


==> sec-oscillator.tex <==
\section{An Illustrative Example} \label{sec:example}
We will show the motivation and introduce our method with a toy example: an underdamped oscillatory system~\cite{gordon2007}, such as a spring-mass or a simple pendulum with a detector that raises an alarm whenever the displacement $x$ exceeds the threshold $a$. The behavior is captured by the following differential equation
\begin{equation}
\frac{\mathrm{d}^2 x}{\mathrm{d}t^2} + \frac{\mathrm{d}x}{\mathrm{d}t} + \omega^2 x = 0
\label{eq:osc}
\end{equation}
with $\omega = 2\pi$. The initial displacement $x(0)=0$, while its tendency to deviate from the equilibrium $x'(0) \in [0,2\pi]$. We are interested in whether the detector will alarm in the first five seconds, i.e., whether there exist a solution $x(t)$ of equation~\eqref{eq:osc} with $x(0)=0$ and $x'(0)\in[0,2\pi]$ such that $x(t) > a$.

%\begin{figure}[t]
%	\centering
%	\scalebox{1.0}{
%		\begin{tikzpicture}[->, node distance = 5cm,scale = 1]
%		\tikzstyle{every node} = [align = center,minimum size = 1.2 cm];
%		\node [initial by arrow,initial text={$x(0)=0$\\$x'(0)\in[0,2\pi]$},initial where = above,state,,minimum size=2.5cm] (INIT){mode $q_0$\\ \\$x''+x'+\omega^2 x = 0$};
%		\node [state,minimum size=2.5cm](T1)[right of = INIT]{mode $q_e$\\ \\$x'=0$};
%		
%		\path
%		(INIT)edge node [above=0.01cm] {$x>a$}(T1);
%		
%		\end{tikzpicture}
%	}
%	\caption{An underdamped oscillatory system } %with a displacement detector
%	\label{fig:osc_automata2}
%\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{image/oscillator.png}
	\caption{Example trajectories}
	\label{fig:oscillator}
\end{figure}

A numeric way to solve the problem is to randomly generate a lot of initial values $v_0^{(i)} \in [0,2\pi]$, and for each $v^{(i)}$ we generate many $t^{(i)}_j\in[0,5]$. For each $t_j$ we calculate a numeric approximation of $x(t^{(i)}_j)$ and see whether it is greater than the threshold~$a$. This method is referred to as random sampling, and has been studied extensively~\cite{Veach1995,benjaminsmc,HypothesisTestingDenise1996,HypothesisTestingTal2011, ReliabilityDemonstrationSharma2010,YounesThesis,Legay2010}.
Random sampling is efficient and scalable, but it fails to find \emph{rare events}, i.e., events that rarely happen. As in Figure~\ref{fig:oscillator}, it is only when the initial displacement is close to $2\pi$ can the system deviate from the equilibrium by more than threshold $a$. Even with such an initial condition, the time window for the displacement to be greater than $a$ is very narrow. As a result, the detector raising an alarm is a rare event, and a rather large number of random samples are required to show its presence.

%\begin{table}
%	\caption{Simulation results}
%	\label{tab:simulation}
%	\begin{tabular}{c|c|c|c|c}
%		\hline
%		Simulation	& 1			& 2			& 3			& 4      	\\ \hline
%		$v_0$		& $3.3094$ 	& $4.7863$ 	& $4.4481$ 	& $4.8553$ 	\\ \hline
%		$t  $ 		& $4.9135$ 	& $1.2455$ 	& $3.7177$ 	& $4.7538$ 	\\ \hline
%		$x(t)$ 		& $-0.0271$	& $0.4094$	& $-0.1064$ & $-0.0718$ \\ \hline
%		$x(t)>a?$	& False		& False		& False		& False		\\ \hline
%		\hline
%		Simulation	& 5			& 6			& 7			& 8      	\\ \hline
%		$v_0$		& $1.8047$ 	& $1.6208$ 	& $0.8966$ 	& $5.6816$ 	\\ \hline
%		$t  $ 		& $3.6641$ 	& $2.2380$ 	& $1.4510$ 	& $2.3685$ 	\\ \hline
%		$x(t)$ 		& $-0.0377$	& $0.0839$	& $0.0229$	& $0.2128$	\\ \hline
%		$x(t)>a?$	& False		&False		&False		&False		\\ \hline
%	\end{tabular}
%\end{table}

%Suppose the first eight random samples of tuples $(v_0,t)$ are as follows~(Table~\ref{tab:simulation}). Unfortunately, they all failed to find the rare event of

An alternative way is to apply analytical methods, such as symbolic execution, to identify a concrete instance $t\in[0,5]$ such that $x(t) > a$ if there is any. Symbolic execution works by constructing a necessary constraint (i.e., path conditions) for certain event to occur and solving the constraint using an SMT solver to show that constraint is unsatisfiable or otherwise. The trouble is that symbolic execution consumes more time and memory, so we would like to apply it only if certain relevant events are rare \emph{enough}. Thus, we always start with random sampling. As the sampling goes on, we become \emph{more and more confident} that the events which have not occurred are rare events, and resort to symbolic execution at certain point.

Take the oscillator as an example. In the beginning, we will estimate the probability of alarming to be $1/2$. Suppose the first eight random samples fail to trigger the rare event $x(t)>a$. We will update the estimation as $(0+1)/(8+0+1) = 1/9$. As a result, the expected cost of random sampling in order to fire this rare event exceeds the cost of symbolic execution. We thus apply symbolic execution, i.e., collecting the following path conditions that triggers an alarm.
 \begin{align*}
         &x''+x'+ \omega^2 x=0 \ \land\  x(0) = 0 \ \land\  0 < x'(0) < 2\pi \\
 \land\  &0 < t < 5                   \ \land\  x(t) > a \land \omega = 2\pi \land a = \pi/4.
 \end{align*}
We use dReal~\cite{gao2013dreal}, a solver for hybrid constraints, to solve it. dReal took $0.024$ seconds to find an instance of~$(v_0,t) = (5.5640, 0.2330)$ such that $x(t) = 0.7858 > a$.

We remark that our method is more effective than random sampling in this example, as we need in average more than four hundreds samples to find a tuple $(v_0,t)$ such that $x(t) > a$, which would take more time. Furthermore, our method is often more cost-effective than applying symbolic execution for every path in the hybrid model, or some combination of random sampling and symbolic execution without considering the probability of system transitions or the cost of symbolic execution.

% compared to only eight simulations plus a single use of dReal in our method.


% In short, our method made eight simulations to tell that the undiscovered transition $q_0\to q_e$ is a rare event, and immediately trigger the analytical tool dReal to solve for a solution. It prevents from using the relatively expensive analytical tools to solve for solutions of trivial common events, and also prevents from countless of random simulations if we meet with rare events.

% The oscillatory example will be used in the following sections as a running example to illustrate important concepts.


==> sec-ourmethod.tex <==
\section{Our Method}\label{sec:implementation}
In this section, we present in detail how our approach works.

\subsection{Problem Definition}
The problem that we aim to solve is that, give a hybrid system model and a property, we would like to find a counterexample efficiently or otherwise be able to conclude that the property is satisfied all the time. In particular, the system models that we are targeting are hybrid automata, which we define formally in the following. As a convention, we use $x_1,x_2,x_3,\dots$ to denote state variables and $q_1,q_2,q_3,\dots$ to denote modes. %For simplicity, we use vector $\vec{x} = (x_1,x_2,\dots)$ to denote all state variables.
A \emph{guard} is a propositional logic formula constituted by propositions on the state variables. The set of all guards over the state variables is denoted as $\G$. Technically speaking, a guard $g \in \G$ specifies the set of valuations of state variables which satisfy $g$.

\begin{definition} A hybrid automaton is a tuple ${\cal H} = (Q,q_{in},V, v_{in}, \to, \{f_q\}_{q\in Q})$ where
\begin{itemize}
	\item $Q$ is a finite set of modes and $q_{in} \in Q$ is the initial mode;
	\item $V = \{x_1,x_2,\dots,x_n\}$ is the set of state variables; $v_{in}$ specified the initial values of the state variables. Without loss of generality, we assume $v_{in}$ specifies that each variable $x_i \in V$ initially satisfies: $l_i \leq x \leq u_i$ where $l_i$, $u_i$ are rational numbers;
	\item $\to \subseteq Q \times \mathcal{G} \times Q$ is a labeled transition relation;
	\item $\{f_q\}_{q\in Q}$ is a set function which associates each mode with a function $f_q$ such that $\mathrm{d}V/\mathrm{d}t = f_q$;
%	\item $L: Q \to 2^{AP}$ associates each mode $q$ with a set of atomic propositions.
\end{itemize}
\end{definition}

A (concrete) \emph{state} $(q,v)$ of ${\cal H}$ is a pair of $(q, v)$ where $q \in Q$ and $v$ is a valuation of $V$. Given a mode $q$, solutions of the equation $\mathrm{d}V/\mathrm{d}t = f_q$ are called \emph{trajectories} in mode $q$. Adopting the convention in the differential equation theory, we use $\Phi_q, \Phi_{q_1}, \Phi_{q_2} \dots$ to denote the \emph{phase space trajectories}. Therefore the trajectory in mode $q$ with initial valuation $v_0$ is $\Phi_q(t,v_0)$. A path of $H$ is a sequence of connected mode changes $\langle (q_0, g_0, q_1), (q_1, g_1, q_2), \cdots \rangle$. A run of $H$ is a sequence of alternating \emph{trajectories} in certain mode and mode changes. In this work, we assume all system runs are \emph{non-Zeno}, i.e., infinity number of mode changes cannot happen within a finite amount of time. We define the length of a run or a path to be the number of mode changes in the run. A path of ${\cal H}$ is feasible if there is a run which has the same sequence of mode changes.

We assume that system properties are expressed in the form of \emph{bounded linear time logic}~(BLTL) formulae. A BLTL formula $\varphi$ is defined as
\[	\varphi::= true \mid false \mid A \mid \lnot \varphi \mid \varphi_1 \land \varphi_2 \mid \varphi_1 \lor \varphi_2
	\mid \varphi_1 \mathbf{U}^{\leq l} \varphi_2,
\]
where $A$ is an atomic proposition, $\varphi_1$ and $\varphi_2$ are BLTL formulae. We remark that other commonly used temporal operators like $\square$ (a.k.a.~always) can be defined using the above operators. Furthermore, for simplicity, we assume that $A$ is always a proposition denoting whether the system is at certain mode. Next, we define what it means to say that ${\cal H}$ satisfies a a BLTL formula $\varphi$, written as ${\cal H} \vDash \varphi$.

Without loss of generality, we assume that there is a unit time step length $\Delta > 0$ such that at most one mode transition could occur within any unit period $\left[n\Delta, (n+1)\Delta\right)$. We thus \emph{discretize} the time domain $\reals_{\ge 0}$ into a set of \emph{observation points} $\{0, \Delta, 2\Delta, \cdots\}$. A run of $H$ thus can be discretized into a trace $\pi= \langle (q_0,v_0),(q_1,v_1),\cdots,(q_n,v_n)\rangle$ where $q_i$ is the mode that the system is relying at at the $i$-th observation point and $v_i$ is the valuation of the state variable at the time. We write $\pi_i$ to denote the suffix of $\pi$ starting with $(q_i,v_i)$. Further, we write $\pi \vDash \varphi$ to denote the $\pi$ satisfies $\varphi$, which is defined as follows: where $false$, $true$, $\lnot$, $\land$ and $\lor$ are interpreted as usual,
\begin{itemize}
\item $\pi \vDash A$ if $q_0 = A$, i.e., the system is at the mode specified by $A$;
\item $\pi \vDash \varphi \mathbf{U}^{\le l} \psi$ if there exists $i$ such that $i \le l$ and $\pi_i \vDash \psi$; and $\pi_j \vDash \varphi$ for all $j$ such that $0 \leq j < i$.
\end{itemize}
We say that a hybrid automata ${\cal H}$ satisfies $\varphi$, denoted as ${\cal H} \vDash \varphi$, if all traces of ${\cal H}$ satisfies $\varphi$. Given $\varphi$, we can compute a constant $K$ which is the maximum number of time steps we need to check whether $\varphi$ is satisfied or not. Furthermore, we can construct a finite-state automaton with at most $K$ states which accepts only counterexample of $\varphi$. As a result, we can effectively reduce the problem of verifying ${\cal H} \vDash \varphi$ to a reachability analysis, i.e., whether an accepting state of the finite-state automaton is reachable in K steps. For simplicity, in the following, we present our approach in the setting of this reachability problem.

\subsection{Step 1: Sampling}
The first step of our approach is to apply the sampling-based method proposed in~\cite{benjaminsmc}. We remark that different from the standard Monte Carlo simulation, the method in~\cite{benjaminsmc} provide a probabilistic guarantee on the absence of counterexample, which is preserved in our method. In the following, we briefly introduce the sampling method and the probabilistic guarantee. Interested readers are referred to~\cite{benjaminsmc} for details.

Algorithm 1 shows the sampling algorithm. It takes a hybrid automaton and a constant $K$ which is the maximum number of step we need to simulate so as to tell whether the formula $\varphi$ is satisfied or not. We remark that as we discussed above, we assume $\varphi$ is a set of modes in ${\cal H}$ such that a feasible path reaching a mode in $\varphi$ is a counterexample. Algorithm 1 returns a sampled trace which is then used to check whether $\varphi$ is violated. Firstly, a state $(q_0, v_0)$ is randomly chosen from the set of initial valuations for the state variables (line 1 and 2). Next, for each step, a set of $J$ (a constant which we will discuss later) time points are randomly picked with a time step. With the time points, we evaluate how many times each outgoing transition from the current mode is enabled. At line 7, we randomly choose a transition accordingly to the likelihood of it being enabled among the selected time points. Once the transition is selected, we randomly take one from the selected time points which enable the transition and then continue system simulation from the state after that transition.

The method in~\cite{benjaminsmc} works by, taking a target probabilistic guarantee $p$ and a confidence $c$ as inputs and using Algorithm 1 to keep sampling the system behaviors until (1) either a trace which fails the given property $\varphi$ is sampled or (2) the number of samples reaches a threshold $N$, which is the number of samples required for the probabilistic guarantee, i.e., the property is satisfied with a probability $p$ and a confidence $c$. While the above method overpasses the difficulty that most ordinary differential equations have no closed form solution but only numeric approximation, there are limitations. Firstly, this probabilistic conclusion could be confusing given that it is based on the assumption that ``\emph{mode transitions in hybrid systems are stochastic events and the probability of a mode transition is proportional to the measure of the value state and time point pairs at which this transition is enabled}''~\cite{benjaminsmc}. Besides, there is the question of how to set $J$, which is used to estimate the probabilistic distribution of the outgoing transitions from a mode. A larger $J$ could generate a better approximation of the actual distribution and would trigger rare events, with the price of more computational cost. In the following, we aim to improve the algorithm to overcome its limitations.

\begin{algorithm}[t]
%\KwData{Automaton $(Q,q_{in},V,v_{in},\to,\{f_q\}_{q\in Q})$; maximum step $K$; property $\varphi$; number $N$}
 \KwResult{a set of traces $\Pi$}
Let $\Pi$ be an empty set of traces; \\
\Repeat {$N$ times} {
Pick a random initial valuation $v_0$; \\
Set $\pi$ to be $\langle (q_0,v_0) \rangle$ where $q_0 = q_{in}$; set $k$ to be 0; \\
\While {$k \leq K$} {
        Sample a set of $J$ time points uniformly from $[0,\Delta]$; \\
        \For {each outgoing transition $t_i = (q_k, g_i, q_i)$ from $q_k$} {
		  Set $T_i:= \{ t \in J \mid \Phi_{q_k}(t,v_k) \in g_i \}$,
        }
		Choose a transition $t_i$ with probability $|T_i| / \left(\sum_i |T_i| \right)$; \\
		Sample a time point $t$ uniformly from $T_i$; \\
		Set $v_{k+1} := \Phi_{q_{k+1}}(1-t, \Phi_{q_k}(t,v_k))$; set $q_{k+1} = q_i$; \\
		Set $\pi := \pi \cdot \langle t_i, (q_k, v_k) \rangle$; \\
}
\If {$\pi$ fails $\varphi$} {
        present $\pi$ as a counterexample and terminate;
    }
Add $\pi$ into $\Pi$;
}
Return $\Pi$
\caption{$Sample(Q,q_{in},V,v_{in},\to,\{f_q\}_{q\in Q}, K, \varphi, N)$}
\end{algorithm}

%
%\begin{theorem}\label{consistence}
%$H \models \varphi$ if and only if $M \models \varphi$.
%\end{theorem}

%\begin{theorem}\label{hypothesis}
%Given $\delta$ and $\alpha$, there exists an $N$ such that testing $N$ times ...
%\end{theorem}



\begin{example}
In the Sewerage System testcase, we want to test two BLTL properties. $\square \neg Recover$ and $\square \neg Shutdown$. For both properties, in step 1, after N samples, we sampled traces of (normal,load,normal) and (normal,drain,normal). We tested the trajectories against the two properties, and is not able to falsify. 
\end{example}

\subsection{Step 2: Symbolic Execution}
Assume first we pick a value for $J$ based on our experience. During the execution of Algorithm 1, certain outgoing transition $t_i = (q_k, g_i, q_i)$ may never be enabled with the selected $J$ time points, during the $k$-th iteration. This could be because that the transition is indeed infeasible from state $(q_k, v_k)$ or it could be that it is a rare event (with respect to the value chosen for $J$). Distinguishing the two systematically would be beneficial as in the former case, we would be able to prove that there is no counterexample taking that transition and in the latter case we may find a counterexample following the transition. In the following, we adopt an idea similar to concolic testing~\cite{sen2006cute} to use an SMT solver to answer the question on whether certain transition/path is feasible or not. The SMT solver we use in our method is \emph{dReal}~\cite{gao2013dreal}.

In particular, if transition $t_i = (q_k, g_i, q_i)$ is never sampled from state $(q_k, v_k)$, we use the solver to check the satisfiability of the formula: $\exists t \mid 0 \leq t \leq \Delta.~\Phi_{q_k}(t,v_k) \Rightarrow g_k$. There are two outcomes. Either it is not satisfiable or \emph{dReal} would return a range of values of $t$ such that the constraint is satisfied. We remark given a path of ${\cal H}$: $P = \langle (q_1, g_1, q_2), (q_2, g_2, q_3), \cdots, (q_n, g_n, q_{n+1}) \rangle$ and a starting state $(q_1, v_1)$, we can solve the following formula to check the feasibility of the path from valuation $v_1$:
\begin{eqnarray*}
\exists t_1, \cdots, t_n, v_2, \cdots, v_n & & \Phi_{q_1}(t_1,v_1) \Rightarrow g_1 \land v_2 = \Phi_{q_2}(\Delta-t_1, \Phi_{q_1}(t_1,v_1)) \\
             & & \land \Phi_{q_2}(t_2,v_2) \Rightarrow g_2 \land v_3 = \Phi_{q_3}(\Delta-t_2, \Phi_{q_2}(t_2,v_2)) \\
             & & \land \cdots \\
             & & \land \Phi_{q_n}(t_n,v_n) \Rightarrow g_n
\end{eqnarray*}
We write $fea(P, v_1)$ to denote a function which solves the above constraint and returns a constraint on $t_1, t_2, \cdots, t_n$ which satisfies the constraint. If the constraint is unsatisfiable, it returns false. Similarly, we define function $fea(P)$ to denote a function which solves the following constraint and returns a constraint on $t_1, t_2, \cdots, t_n$ which satisfies the constraint: $\exists v1.~fea(P, v_1)$. We remark that function $fea(P)$ checks the feasibility of the path from any variable valuation. In theory, we can use the solver to check the feasibility of every path which potentially constitutes a counterexample. Solving such path constraints involving ODEs is however rather complicated. Thus, we develop an approach which favor local proofs which show infeasibility of certain path.

\begin{algorithm}[t]
\KwData{Run $\pi = \langle (q_0,v_0), (q_1,v_1), \cdots, (q_k,v_k)\rangle$; transition $(q_k, g_k, q_{k+1})$; set of paths $Inf$}
\KwResult{a new trace or $null$}
Set $i := k$; $P := \langle (q_k, g_k, q_{k+1}) \rangle$; $result := \langle \rangle$; \\
\While {$P \not \in Inf$ and $i \geq 0$} {
        \If {$fea(P, v_k)$ does not return false} {
%            $result := result \cdot \langle fea(P, v_k) \rangle$; \\
            \Return a trace $\pi'$ which has the same sequence of transitions as $\pi$ and takes transition $(q_k, g_k, q_{k+1})$ as its last step;
        }

        \If {$fea(P)$ returns false} {
            Add $P$ into $Inf$;\\
            \Return $null$;
        }
    	Set $i := i-1$; $P := \langle (q_i, g_i, q_{i+1}) \rangle \cdot P$;
}
\Return $null$;
\caption{$Solve(\pi, q_k, g_k, q_{k+1}, Inf)$}
\end{algorithm}

If a transition $(q_k, g_k, q_{k+1})$ is never sampled after step $k$, and furthermore, by a simple analysis, following the transition from the current trace $\pi$ may potentially lead to a counterexample, Algorithm 2 is invoked so as to check whether the transition is indeed infeasible. Algorithm 2 takes as input the transition, a path $\pi$ and a set of paths $Inf$ which are known to be infeasible (i.e., for all $h \in Inf$, $fea(h)$ returns false). First, at line 3, we try to see whether the transition is feasible from the last state in $\pi$. If it is, we return the constraint for later steps. Otherwise, we check at line 5 whether the transition is feasible with any variable valuation at mode $q_k$. If it is negative, we add it into $Inf$ and return false. Otherwise, we continue the loop to look back for one more step. The loop terminates either when we find a sequence of constraints which makes the transition feasible or find that it is infeasible.


%It can handle formulas in the framework of $\delta$-complete decision procedure
%\footnote{SMT formulas are hard to verify when nonlinear functions are involved. In the framework of $\delta$-complete decision procedure, a decision procedure is said to be $\delta$-complete if for any $\varphi$ from set $S$ of SMT formulas the procedure returns below answers:\\
%$\cdotp$ unsat: $\varphi$  is unsatisfiable.\\
%$\cdotp$ $\delta$-sat: $\varphi^{\delta}$ is satisfiable.\\
%If we take a look at $\varphi^{\delta}$, $\delta$ is a user specified positive real number meant for a  mathematical relaxation on the original $\varphi$. With this relaxation, dReal improve numerical algorithms' efficiency for nonlinear problems and provide correctness guarantees at the same time.

% On the other hand, \emph{Symbolic execution} is able to cover more states of a program by not giving any specific values to variables but only recording constraints on variables along the execution paths, e.g. constraints from condition statement {\sf if} and {\sf switch}. It also provides a guideline for systematically examining the branches. With powerful SMT solvers \cite{platzer2010logical,gao2014delta,henzinger1997hytech}, symbolic execution is able to determine if an execution path is reachable or not, but it does not work well in large programs for its high time consumption.
%
%\emph{Concolic testing} combines random testing and symbolic execution. It starts with symbolic execution and explore branches of a program in a systematical way. While it fails to reach some specific states, it resorts to random testing until the expected states are discovered. We borrow the idea of concolic testing in our method for probabilistic hybrid system verification. As in Fig. \ref{guardcovery}, the vector with color represents guard. The guard in black means covered at least once and the color red means the guard is never satisfied. Now we find that in trajectory $1$, only state $B$ was covered. In trajectory $2$, only $C$ was covered. In trajectory $3$, $B$ and $C$ were both covered, leaving only $D$ uncovered. Note that in this case, we only check the guard $D$'s satisfiability for all $3$ trajectories but not $B$ or $C$, as they were covered at least once in all trajectories.

%\iffalse
%Figure~\ref{guardcovery} shows an example when we explore the modes of a hybrid system. Firstly, we use inexpensive numerical ODE solvers to find when mode guards are satisfied, and we will cover $mode$ 1, 2 and 4 in short time. After exploring some time we find that  $mode\ 3$ can't be traversed, so we adopt SMT solvers to check if $mode \ 3$ is reachable. If it is then SMT solvers will tell us under which circumstances can we reach $mode\ 3$, and we will explore from $mode \ 3$ using numerical ODE solvers again, until we explore all reachable modes.
%\fi
%
%
%\begin{figure}
%\centering
%\scalebox{0.6}{
%\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
%\clip(-1.,-1.5) rectangle (8.,9);
%\draw(2.5,7.5) circle (0.5cm);
%\draw(2.5,4.) circle (0.5cm);
%\draw(2.5,0.5) circle (0.5cm);
%\draw(5.,8.5) circle (0.5cm);
%\draw(6.,7.5) circle (0.5cm);
%\draw(5.,6.5) circle (0.5cm);
%\draw(5.,5.) circle (0.5cm);
%\draw(6.,4.) circle (0.5cm);
%\draw(5.,3.) circle (0.5cm);
%\draw(5.,1.5) circle (0.5cm);
%\draw(6.,0.5) circle (0.5cm);
%\draw(5.,-0.5) circle (0.5cm);
%\draw [->] (3.,7.5) -- (4.5,8.5);
%\draw [->,color=ffqqqq] (3.,7.5) -- (5.5,7.5);
%\draw [->,color=ffqqqq] (3.,7.5) -- (4.5,6.5);
%\draw [->,color=ffqqqq] (3.,4.) -- (4.5,5.);
%\draw [->] (3.,4.) -- (5.564028409036256,3.997786611430251);
%\draw [->,color=ffqqqq] (3.,4.) -- (4.5,3.);
%\draw [->] (3.,0.5) -- (4.5,1.5);
%\draw [->] (3.,0.5) -- (5.5,0.5);
%\draw [->,color=ffqqqq] (3.,0.5) -- (4.5,-0.5);
%\draw (2.1093331114506507,7.739149125589634) node[anchor=north west] {$A_1$};
%\draw (2.0840923560318448,4.243304500085007) node[anchor=north west] {$A_2$};
%\draw (2.0840923560318448,0.7727006299991874) node[anchor=north west] {$A_3$};
%\draw (4.557686387074805,8.761399720051276) node[anchor=north west] {$B_1$};
%\draw (5.567316603827034,7.739149125589634) node[anchor=north west] {$C_1$};
%\draw (4.570306764784208,6.79262079738441) node[anchor=north west] {$D_1$};
%\draw (4.557686387074805,5.252934716837246) node[anchor=north west] {$B_2$};
%\draw (5.567316603827034,4.29378601092262) node[anchor=north west] {$C_2$};
%\draw (4.582927142493611,3.309396549589187) node[anchor=north west] {$D_2$};
%\draw (4.570306764784208,1.731849335913814) node[anchor=north west] {$B_3$};
%\draw (5.567316603827034,0.7853210077085905) node[anchor=north west] {$C_3$};
%\draw (4.570306764784208,-0.23692958675305117) node[anchor=north west] {$D_3$};
%\begin{scriptsize}
%\draw [fill=qqqqff] (1.5,7.5) circle (1.5pt);
%\draw [fill=qqqqff] (1.,7.5) circle (1.5pt);
%\draw [fill=qqqqff] (0.5,7.5) circle (1.5pt);
%\draw [fill=qqqqff] (0.,7.5) circle (1.5pt);
%\draw [fill=qqqqff] (1.5,4.) circle (1.5pt);
%\draw [fill=qqqqff] (1.,4.) circle (1.5pt);
%\draw [fill=qqqqff] (0.5,4.) circle (1.5pt);
%\draw [fill=qqqqff] (0.,4.) circle (1.5pt);
%\draw [fill=qqqqff] (1.5,0.5) circle (1.5pt);
%\draw [fill=qqqqff] (1.,0.5) circle (1.5pt);
%\draw [fill=qqqqff] (0.5,0.5) circle (1.5pt);
%\draw [fill=qqqqff] (0.,0.5) circle (1.5pt);
%\end{scriptsize}
%\end{tikzpicture}
%}
%\caption{The Hybrid Concolic Guard Covering}\label{guardcovery}
%\end{figure}
%
%\iffalse
%\begin{figure}
%\centering
%\scalebox{1.3}{
%\begin{tikzpicture}
%	\tikzstyle{every node} = [align = center,text width=3mm];%minimum size = 0.2 cm];
%	\node [initial,state] (INIT){$INIT$};
%	\node [state](T1)[above left of = INIT]{$mode\ 1$};
%	\node [state](T2)[above of = INIT]{$mode\ 2$};
%	\node [state,draw=red](T3)[above right of = INIT]{$mode\ 3$};%this is a rare mode
%	\node [state](T4)[right of = INIT]{$mode\ 4$};
%	\node [state](T5)[above of = T3]{$mode\ 5$};
%	\node [state](T6)[above right of = T3]{$mode\ 6$};
%	\node [state](T7)[right of = T3]{$mode\ 7$};
%	\node [state,draw=red](T8)[above right of = T7]{$mode\ 8$};%this is a rare mode
%	\node [state](T9)[below right of = T7]{$mode\ 9$};
%	\path
%		(INIT)edge[]node {}(T1)
%		(INIT)edge[] node {}(T2)
%		(INIT)edge[] node {}(T3)
%		(INIT)edge[] node {}(T4)
%		(T3)edge[] node {}(T5)
%		(T3)edge[] node {}(T6)
%		(T3)edge[] node {}(T7)
%		(T7)edge[] node {}(T8)
%		(T7)edge[] node {}(T9);
%\end{tikzpicture}
%}
%\caption{Concolic testing in mode exploration}
%	\label{concolic_checking}
%\end{figure}
%\fi

\begin{example}
Reviewing the trajectories, we find that guard $(normal,g,flooding)$ is neverd covered so we call dreal to solve it. And we find that there is a small region in time domain to make the guard satisfiable.
For trajectory (normal,flooding), we find that no sample is able to extend the trajectory. We use dreal and fail to cover either. So we trace back to node $normal$, and solved (normal, flooding, recover) and (normal, flooding, shutdown), we find that only (normal,flooding,recover) is feasible, so we put (normal, flooding, shutdown) to feasible.
\end{example}

%\subsection{Step 3: Importance Sampling}
%After the previous steps, we have sampled the system with a particular sample rate (i.e., the number of $J$ time point) and we have identified some constraint which could help me \emph{trigger} some paths which have not been sampled. Next, we use constraint and apply the idea of importance sampling. In the following, we briefly introduce the idea of importance sampling.
%
%In Algorithm 1, we estimate the probability distribution of all outgoing transitions from a mode (with certain variable state) using Monte Carlo simulation. It is straightforward to see that when $J$ converges to $\infty$, the estimation converges to the actual distribution.
%%%%sunjun: the following hasn't been modified as I can't make sense out of it; make sure every notation is explained properly before using it. Make sure an example is used to explain every nontrivial construciton.
%However, due to limited computing resource, we have an upper bound $B_r$ on sample rate. There's common situations when we need to use Monte Carlo's method to estimate $E(f(x))$ according to $P(X)\sim X$. While the value $f(x)$ on $A\subseteq X$ is significantly larger than that on $A^C$. Or when we use fixed sample rate while $f(x)$ is a periodic function where its period equals to sample period. In these situations, we need to introduce the so-called \emph{importance sampling} method.
%The basic idea is to replace the original normal distribution with new probability distribution $Q(X)\sim X$, while maintain our desired expectation value $E_p(f(x))$. As depicted in Eq.\ref{normalsample} based on normal distribution and Eq.\ref{importancesample} based on importance sampling, it is easy to tell that $E_p(f(x))=E_q(\frac{f(x)p(x)}{q(x)})$.
%
%\begin{equation}\label{normalsample}
%E_p(f(x))=\int \! f(x)p(x)\mathrm{d}x
%\end{equation}
%
%\begin{equation}\label{importancesample}
%E_q(\frac{f(x)p(x)}{q(x)})=\int \! \frac{f(x)p(x)}{q(x)}q(x)\mathrm{d}x
%\end{equation}
%Needless to say that the new distribution $Q(X)\sim X$ should also satisfy that $\int \! q(x)\mathrm{d}x=1$, while the sample rate on $A$ should exceed that on $A^C$ for $Q(X)\sim X$. Next we have our importance sampling estimate with $n$ samples given in Eq.\ref{im_sam_estimate}.
%
%\begin{equation}\label{im_sam_estimate}
%\hat{\mu}_q=\frac{1}{n}\sum_{i=1}^{n} \frac{f(x_i)p(x_i)}{q(x_i)}, x_i\sim q
%\end{equation}
%
%We thus have the $E_q(\hat{\mu}_q)=\mu$, and we have
%\begin{equation}
%\sigma_q^2=\int \! \frac{(f(x)p(x))^2}{q(x)}q(x)\mathrm{d}x-\mu^2
%\end{equation}
%
%As a good sample $Q(X)\sim X$ is with a smaller $\sigma_q^2$, and $\mu$ is set, we need to get a smaller $\int \! \frac{(f(x)p(x))^2}{q(x)}q(x)\mathrm{d}x$. We will introduce our design of $Q(X)\sim X$ in Sec. \ref{subsectionimportancesampling}.
%
%
%After finding the importance region $A\subset (0,1)$, we will adjust our sampling from $ N(t)\sim t$ to $ R(t)\sim t$.
%Recall in Eq. \ref{probabilitypropagation} we had the inner integration based on $T_j(\vec{v})$, now we do some modification on this equation. We note that the value of indicator function $1_Z$ equals to $0$ for any $t\notin T_j(\vec{v})$, so we can equally change our integration region to $(0,1)$. Then we propose our importance sampling distribution as given in Eq. \ref{rt}.
%
%\begin{equation}\label{rt}
%R(t)=
% \begin{cases}
%      \frac{a}{(a-1)\mu(A)+\mu(B)} & t \in A \\ \\
%      \frac{1}{(a-1)\mu(A)+\mu(B)}  & t \notin A
%   \end{cases}
%\end{equation}
%
%Here $a$ represents the ratio of sampling rate for $t\in A$ compared to that where $t\notin A$. And $(a-1)\mu(A)+\mu(B)$ is a normalization factor to make $\int_{0}^1 \! R(t) \mathrm{d}t=1$. And so we can reform the integration as shown in Eq. \ref{newdistripropa}. it is easy to tell that Eq. \ref{probabilitypropagation} and Eq. \ref{newdistripropa} are equivalent.
%
%\begin{equation}\label{newdistripropa}
%P_{X_j}(Y)= \int_{\vec{v} \in X} \int_{t\in (0,1)} \! \frac{1_{(\Phi_{q_j}(1-t,\Phi_{q}(t,v))\bigcap Y}N(t)}{R(t)} \mathrm{d}R(t) \mathrm{d}P(X)
%\end{equation}
%
%Here $N(t)$ is our the nominal distribution, $R(t)$ is the importance distribution and the adjustment factor $N(t)/R(t)$ is called the likelihood ratio. We can see that $N(t)=1$ for any $t\in (0,1)$, so we can shorten Eq. \ref{newdistripropa} to get Eq. \ref{rtshorten}.
%
%\begin{equation}\label{rtshorten}
%P_{X_j}(Y)= \int_{\vec{v} \in X} \int_{t\in (0,1)} \! \frac{1_{(\Phi_{q_j}(1-t,\Phi_{q}(t,v))\bigcap Y}}{R(t)} \mathrm{d}R(t) \mathrm{d}P(X)
%\end{equation}
%
%And so we will sample the value of $\frac{1_{(\Phi_{q_j}(1-t,\Phi_{q}(t,v))}}{R(t)}$ according to $R(t)\sim t$ and get $E_r(\frac{1_{(\Phi_{q_j}(1-t,\Phi_{q}(t,v))}}{R(t)})$ for the inner integration.
%
%\begin{example}
%Here we show how this step works for the sewerage system.
%\end{example}

\subsection{Overall Algorithm}
In the following, we present the overall algorithm, shown as Algorithm \ref{mainalgri}, and discuss its properties. Firstly, we identify the set of all modes which could reach a mode in $\varphi$. Intuitively, we could skip ignore paths visiting modes not in the set since they would never constitute a counterexample. At line 2, we apply Algorithm 1 to sample traces based on~\cite{benjaminsmc}. Afterwards, we check whether, after $k$ steps, there is a transition which is never sampled (and could lead to a counterexample). If there is, for each path from the initial mode to the current mode, we pick a representative from the set of sampled traces and apply Algorithm 2 to check whether it is feasible to enable the transition. If it is not feasible, we continue with a different path. Otherwise, we apply Algorithm 1 to sample traces which extends the trace returned by Algorithm 2. The algorithm terminates whenever a counterexample is sampled through an invocation of Algorithm 1. Else, it concludes that the property is satisfied at line 13. 


%%%sunjun: we need to establish theorems to say that Thiagu's conclusion hold in our setting and if we return no counterexample by letting L to be K, there is no counterexample.
The following establishes the correctness of our method. 
\begin{theorem}
Algorithm~\ref{mainalgri} returns true if and only if the property is satisfied. \hfill \qed
\end{theorem}
We sketch the proof as follows. We can show that the following loop invariant holds for the loop in Algorithm~\ref{mainalgri}: for any path of ${\cal H}$ from $q_{in}$ such that its length is $k$ which ends with a mode in $Q_{bad}$, either it is infeasible or there is at least one run sampled in Algorithm 1 which has the same sequence of first $k$ mode changes. Thus, if there is a counterexample, it must be reported in Algorithm 1 (since all runs are checked there). Therefore, the above theorem holds. The following establishes the completeness of the algorithm. 

\begin{algorithm}[t]
% \KwData{Automaton $H = (Q,q_{in},V,v_{in},\to,\{f_q\}_{q\in Q})$; maximum step $K$; threshold $J$; property $\varphi$}
 \KwResult{a trace $\pi$}
Let $Q_{bad}$ be the set of modes from which there is a path to any mode in $\varphi$;\\
Let $\Pi$ := $Sample(Q,q_{in},V,v_{in},\to,\{f_q\}_{q\in Q}, K, \varphi, N)$\;
set $k$ to be 0; $Inf$ to be an empty set; \\
\While {$k \leq K$} {
        Let $Q_k$ be the set of modes visited by traces in $\Pi$ at step $k$;\\
          \For {each transition $(q_{k-1}, g, q)$ s.t.~$q_{k-1} \in Q_{k-1}$ and $q \in Q_{bad} \setminus Q_k$} {
            \For {each path from $q_{in}$ to $q_{k-1}$} {
                Pick a run $\pi$ from $\Pi$ which follows the sequence; \\
                Let $\pi'$ := $Solve(\pi, q_{k-1}, g, q, Inf)$;\\
                \If {$\pi'$ is not null} {
                    Let $\Pi'$ := $Sample(Q,q,V,v',\to,\{f_q\}_{q\in Q}, K, \varphi, N)$ where $v'$ is the last variable valuation in $\pi'$\;
                    Attach $\pi'$ to the front of each trace in $\Pi'$ and add it into $\Pi$;
                }
        }
    }
}
\Return true;
\caption{HyChecker($Q,q_{in},V,v_{in},\to,\{f_q\}_{q\in Q}, K, J, \varphi$)}
\label{mainalgri}
\end{algorithm}

%%%sunjun: what is the use of the internal loop on i?
%\begin{algorithm}
% \KwData{Hybrid automaton $H=(Q,q_{in},V,INIT,f,G)$, maximum time step $K$}
% \KwResult{Trajectory $\tau_0,...,\tau_{n-1}$}
% Initialization\;
% Sample n points $v_0$...$v_{n-1}$ uniformly from $INIT$\;
%\For {k:=1,...,K} {
%	\For{i:=0,...,(n-1)}{
%                   Generate time points $T:=t_1,...,t_J$ uniformly in $(0,1)$\;
%		  Simulate $v_i^j:=\Phi_{q_{i}^{k-1}}(t_j,\vec{v}_{i}^{k-1}),\ for\ j\in \lbrace 1,...,J\rbrace$\;
%		  Let $\hat{T}_j:=\lbrace t\in T\ :\ \vec{v}_i^j \in g_j\rbrace$ be the time points where $g_j$ is enabled\;
%	}
%	\If {there are outgoing guards that are never satisfied}{
%		call dReach to check whether they could be satisfied\;
%		\If{sat}{
%			return importance region\;		
%		}
%		\Else
%			{do nothing}
%		Importance sampling according to importance region to get $\hat{T}_{rare}$\;
%	}
%	\For{i:=0,...(n-1)}{
%		Pick $g_l$ randomly according to probability $\lbrace p_j\ :=\ \mid\hat{T}_j \mid / (\sum_{u=1}^{m}\mid \hat{T}_u \mid + \mid \hat{T}_{rare} \mid )\rbrace$\;
%		Pick $t_l$ uniformly at random from $\hat{T}_l$\;
%		Simulate $\vec{v}_{i}^\prime := \Phi_{q_{i}^\prime}(1-t_l,\vec{v}_{i}^l)$, where $q_{i}^\prime$ is the target of $g_l$\;
%		Set $q_{i}^k\ := \ q_{i}^\prime ,\ \vec{v}_{i}^k\ := \ \vec{v}_{i}^\prime$, and extend $\tau_i\ :=\ (q_{i}^0,\vec{v}_{i}^0)...(q_{i}^k,\vec{v}_{i}^k)$\;
%	}
%
%}
%return $\tau_0,...,\tau_1$ for BLTL checking\;
%
%\caption{SMChecker Procedure}
%\label{mainalgri}
%\end{algorithm}

\begin{theorem}
Assume function $fea(H, v_1)$ and $fea(H)$ always terminate, Algorithm~\ref{mainalgri} is always terminating. \hfill \qed
\end{theorem}
This is trivially proved as the number of paths with length $K$ or less are finite. What is perhaps interesting are the order in which the paths are explored. We would first sample those paths which have high probability (without any rare event) and then those paths which are not sampled due to its first mode change is rare and then those paths which start with two rare mode changes and etc. That is, paths are sampled in the decreasing order of their likelihood. 
%%%sunjun: we need to argue this is very beneficial. In fact, we should prove that users can stop Algorithm~\ref{mainalgri} anytime and yet we can provide some probabilistic guarantee on the correctness of the proerty. 

\begin{example}
%%%these part needs to be written after experiments are done
In the sewerage system example, K is chosen to be $2$, N is chosen to be 100. At first, 100 trajectories are sampled. But at $k=1$, guard (normal,g,flooding) was never satisfied. So our algorithm calls dreal to solve out. The algorithm find a satisfiable time region and we expand the set of the trajectory. Then, we extend the trajectory after flooding. We easily sampled the trajectory (normal,flooding,shutdown), but failed to sample (normal, flooding, recover). We called dreal to solve the satisfiability of (flooding,g,recover), but it returns unsat. We thus test for all value states in mode flooding, and solve out the constraint needed to satisfy (flooding,g,recover). We then trace back to mode normal, and solve out the constraint needed for (normal,g,flooding), we find out that the intersection of the two constraints are empty set. We thus add recover to $Inf$. 
\end{example}





















==> sec-probabilistic.tex <==
\section{Probabilistic model checking}\label{sec:prob}%this paragraph is for the probabilistic model checking

The main difficulty in analyzing hybrid systems is to find when guards are satisfied and mode transitions are made. For example, a hybrid automata $H$ initially at evaluation $v$ may take some mode transitions within the time region $[0,\Delta]$. Let us assume that the automata $H$ is able to jump to mode $q_i$ for $i \in \{1,2\}$ when in the time region $\mathbb{T}_i(v) = [0,\Delta] \cap \{t \colon \Phi_q(t,v) \in g_i\}$. In most cases, set $\TT_i(v)$ has no closed form and cannot be manipulated directly, so we changed our point of view. Rather than imaging that automaton $H$ is \emph{running} for one time unit, we slide over all events that happen in $(0,\Delta)$ and only focus on the $\emph{destination}$ that $H$ arrives by the end of one time unit. We know for sure that the automaton $H$ makes exactly one\footnote{We do not sweep off the possibility when $H$ does not make a mode transition in $[0,\Delta]$. We can easily handle this by letting $H$ make a self-transition.} mode transition in $[0,\Delta]$; it either jumps to $q_1$ at some time in $\TT_1(v)$ or jumps to $q_2$ at some time in $\TT_2(v)$, so we \emph{assume} that $H$ takes the $i$th mode transition with probability
$p_i(v) = \mu(\TT_i(v)) / \left(\mu(\TT_i(v)) + \mu(\TT_i(v))\right)$. Here we use $\mu$ to denote the measure of a set.
Notice that the automaton $H$ will destine at evaluation
$\Phi_{q_i}(1-t,\Phi_q(t,v))$ if it makes a mode transition to $q_i$ at some time $t \in \TT_i(v)$, so by taking the $i$th mode transition $H$ will arrive at some evaluation in $X_i(v) = \bigcup_{t \in \TT_i(v)} \Phi_{q_1}(1-t,\Phi_q(t,v))$.

Now we move further and let $H$ start from not a particular evaluation $v$ but a region $X \subseteq \reals^n$. From the similar reasoning we can show that $H$ will destine in $X_i = \bigcup_{v \in X} X_i(v)$ by taking the $i$th mode transition at some time within $[0,\Delta]$ with probability $p_i = \int_{v \in X} p_i(v) \mathrm{d}\PP_X(v)$.

In this way we may \emph{abstract} the behavior of $H$ by describing only its ``region transitions'', e.g. $X \to X_i$ with probability $p_i$. In other words, we abstract $H$ by giving a corresponding \emph{Markov chain}.


%A useful way is to Markov chains are transition systems where the state propagation is a stochastic event. A discrete-time Markov chain is a state transition system, while unlike decidable transition systems, the state change happens stochastically. Given a current state, the future state is traversed based on a certain probability distribution. Below is the formal definition of Markov Chain.

%The first step of our approach is to systematically sample behaviors of a hybrid system model and estimate the probability of satisfying the property based on hypothesis testing.

%The basic idea in \cite{benjaminsmc} is to consider mode transitions in the hybrid automata models as stochastic events and build a Markov Chain accordingly. By hypothet testing of generated trajectories of this Markov Chain, we can tell if $M \vDash \psi$. According to Theorem \ref{mainresulttiago}, which is the main result in \cite{benjaminsmc}, the test result whether $H \vDash \psi$.

%\begin{theorem}\label{mainresulttiago}
%$H \vDash \psi$ iff $M \vDash \psi$
%\end{theorem}
%The Markov Chain is established using a probability propagation method. Let's start from $INIT$ in $q_{in}$, assume we pick random points on $INIT$ according to normal distribution. Other distributions could also be adopted, this is for simplicity purpose. Then for every point we pick, we sample from $(0,1)$ on time $T$ and use numerical solvers like ODE23, ODE45 to calculate the state, and then test them according to outgoing mode guards and then generate the state on time $1$ according to the new mode characteristics. Then we do integration for every picked points on $INIT$ to get a new probability distribution on each possible outgoing modes. Then we carry on this method to generate a Markov Chain accordingly.

%\begin{equation}\label{probabilitypropagation}
%P_{X_{j}}(Y)=\int_{v\in X}\int_{t\in T_j(v)} \! 1_{(\Phi_{q_j}(1-t,\Phi_{q}(t,v))\bigcap Y)}  \mathrm{d}P_{T_{j}(v)}\mathrm{d}P(X)
%\end{equation}

%As Eq. \ref{probabilitypropagation} suggests, where $P_X$ is the probability distribution in original mode, $T_j(\vec{v})$ given in Eq. \ref{tjv} and $g_j$ is the set of all states that would satisfy mode $j$, and $1_Z$ is the indicator function of set $Z$.

%\begin{equation}\label{tjv}
%T_{j}(\vec{v})=\lbrace t \  \vert \ \Phi_{q}(t,\vec{v})\in g_j \rbrace
%\end{equation}

%As depicted in Fig. \ref{markovtree} for the markov chain, every node in this tree structure only has one father, while allowed to have multiple children. The transition probability is calculated in Eq. \ref{transitionprobability}. In this equation, $\mu(T_j(\vec{v}))$ is the measure of $T_j(\vec{v})$.

%\begin{equation}\label{transitionprobability}
%p_j=\int_{\vec{v}\in X}\! \frac{\mu(T_j(\vec{v}))}{\sum_{l=1}^{m}\mu (T_l(\vec{v}))}\mathrm{d}P(X)
%\end{equation}

%The behavior of $H$ and $M$ are depicted using bounded linear-time temporal logic (BLTL), this work is able to handle formulas like $\psi$, $\psi^{\prime}$, $F^{\leq l}\psi$, $G^{\leq l}\psi$, $\psi U^{\leq l}\psi^{\prime}$.

\subsection{Notations}
We formalize the above idea by the following definition.
\begin{definition}[Markov chains]\label{def:mc}
Let $H = (Q,q_{in},V,\{f_q\}_{q\in Q},INIT,\to, L)$ be a hybrid automaton. The Markov chain generated from automaton $H$ is a tuple
$M = (S,P, \eta_0)$ where
\begin{itemize}
	\item $S$ is a set of states and $\eta_0 \in S$ is the initial state;
	\item $P : S \times S \to [0,1]$ is the transition probability function with $\sum_{s'\in S}P(s,s') = 1$ for any state $s,s' \in S$.
\end{itemize}

Each state $\eta \in S$ has the form $(\rho, X, \PP_X)$ where $\rho$ is a finite sequence of modes in $Q$, and $(X, \PP_X)$ is a probability space on $X \subseteq \reals^n$. The initial state $\eta_0 = (q_{in}, INIT, \PP_{INIT})$. {\HC} chooses the uniform distribution as the initial distribution $\PP_{INIT}$. Other probability distributions are also feasible. Further research will disclose how different distributions affect the result.

The transition probability function $P$ is defined as follows. Suppose $\mu = (\rho,X,\PP_X) \in S$ is a state where the sequence $\rho = \dots q$ ends with mode $q$. Mode $q$ has $m$ outgoing transitions $q \xrightarrow{g_l} q_l$ for $1 \le l \le m$. Each transition $q \xrightarrow{g_l} q_l$ induces a probability transition from $\mu$ to $\mu_l = (\rho q_l,X_l,\PP_{X_l})$ where
\begin{itemize}
	\item $X_l = \bigcup_{v \in X}\bigcup_{t \in \TT_l(v)} \Phi_{q_l}(1-t,\Phi_q(t,v))$;
	\item $\PP_{X_l}(Y) = \int_{v \in X}\int_{t \in \TT_l(v)} \left[\Phi_{q_l}(1-t,\Phi_q(t,v)) \in Y\right] \mathrm{d}t \mathrm{d}\PP_X(v)$;
	\item $P(\mu,\mu_l) = \int_{v \in X} \mu(T_l(v))\big/\sum_{i=1}^{m}\mu (T_l(v))\  \mathrm{d}\PP_X(v)$.
\end{itemize}
\end{definition}


%Take Fig.\ref{markovchain}  for an example, we can select state \emph{eat} as our initial state, then the next state could be anyone among \emph{rest}, \emph{jog}, \emph{play} based on their transition probability. Note that the sum of the probability values of the edges coming out of the same node should equal to $1$.

%\begin{figure}
%\centering
%\scalebox{0.7}{
%\begin{tikzpicture}[->, node distance = 3cm,scale = 1]
%	\tikzstyle{every node} = [align = center,minimum size = 3 cm];
%	\node [state] (INIT){eat};
%	\node [state](T1)[right of = INIT]{rest};
%	\node [state](T2)[below of = INIT]{play};
%	\node [state](T3)[right of = T2]{jog};
%	\path
%		(INIT)edge[bend left]node {0.6}(T1)
%		(INIT)edge[bend right] node {0.3}(T2)
%		(INIT)edge[] node {0.1}(T3)
%		(T1)edge[] node {0.8}(T3)
%		(T1)edge[] node {0.2}(INIT)
%		(T2)edge[] node {0.25}(T3)
%		(T2)edge[] node {0.75}(INIT)
%		(T3)edge[bend left] node {0.3}(T2)
%		(T3)edge[bend right] node {0.7}(T1);
%\end{tikzpicture}
%}
%\caption{Simple example of Markov chain}
%	\label{markovchain}
%\end{figure}

We write $\mu \to \mu'$ if $P(\mu,\mu') > 0$.
A \emph{path} of $M$ is a finite sequence of states $\pi = \mu_0\mu_1\cdots\mu_n$ where $\mu_i \to \mu_{i+1}$ for $0 \le i < n$.


